Can Large Language Models Explain Themselves? A Study of LLM-Generated Self-Explanations

Large language models (LLMs) such as ChatGPT have demonstrated superior performance on a variety of natural language processing (NLP) tasks including sentiment analysis, mathematical reasoning and summarization. Furthermore, since these models are instruction-tuned on human conversations to produce "helpful" responses, they can and often will produce explanations along with the response, which we call self-explanations. For example, when analyzing the sentiment of a movie review, the model may output not only the positivity of the sentiment, but also an explanation (e.g., by listing the sentiment-laden words such as "fantastic" and "memorable" in the review). How good are these automatically generated self-explanations? In this paper, we investigate this question on the task of sentiment analysis and for feature attribution explanation, one of the most commonly studied settings in the interpretability literature (for pre-ChatGPT models). Specifically, we study different ways to elicit the self-explanations, evaluate their faithfulness on a set of evaluation metrics, and compare them to traditional explanation methods such as occlusion or LIME saliency maps. Through an extensive set of experiments, we find that ChatGPT's self-explanations perform on par with traditional ones, but are quite different from them according to various agreement metrics, meanwhile being much cheaper to produce (as they are generated along with the prediction). In addition, we identified several interesting characteristics of them, which prompt us to rethink many current model interpretability practices in the era of ChatGPT(-like) LLMs.

==> tables/quant_table.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparison between the self-explanation generated by ChatGPT and traditional explanations computed on it.}
    \label{tab:result-table}
    \begin{tabular}{r|ccccc|ccccc}\toprule
         & \multicolumn{5}{c|}{E-P (Accuracy: 85\%)} & \multicolumn{5}{c}{P-E (Accuracy: 88\%)}\\
         & Comp $\uparrow$ & Suff $\downarrow$ & \dfmit{} $\uparrow$ & \dffrac{} $\downarrow$ & \rankdel{} $\uparrow$ & Comp $\uparrow$ & Suff $\downarrow$ & \dfmit{} $\uparrow$ & \dffrac{} $\downarrow$ & \rankdel{} $\uparrow$ \\\midrule
         Occlusion & 0.15 & 0.26 & \textbf{0.18} & 0.57 & \phantom{-}\textbf{0.00} & 0.20 & 0.23 & \textbf{0.14} & 0.64 & -0.02 \\
         LIME & 0.17 & \textbf{0.22} & 0.13 & \textbf{0.50} & -0.02 & \textbf{0.27} & \textbf{0.20} & 0.10 & \textbf{0.56} & \phantom{-}\textbf{0.02} \\
         \selfexp{} & \textbf{0.19} & 0.25 & 0.16 & 0.55 & -0.03 & \textbf{0.27} & 0.22 & 0.07 & \textbf{0.56} & -0.01 \\\bottomrule
    \end{tabular}
\end{table*}

\begin{table}[t]
    \centering
    \caption{Comparison of all methods with the \topk{} explanations on \topk{}-adapted metrics.}
    \label{tab:result-table-topk}
    \begin{tabular}{r|ccc|ccc}\toprule
         & \multicolumn{3}{c|}{E-P (Accuracy: 0.80)} & \multicolumn{3}{c}{P-E (Accuracy: 0.83)}\\
         & Comp@$k$ $\uparrow$ & Suff@$k$ $\downarrow$ & \dfmit{}@$k$ $\uparrow$ & Comp@$k$ $\uparrow$ & Suff@$k$ $\downarrow$ & \dfmit{}@$k$ $\uparrow$ \\\midrule
         Occlusion & 0.16 & 0.34 & 0.29 & 0.11 & 0.29 & 0.17 \\
         LIME & \textbf{0.17} & 0.28 & \textbf{0.40} & \textbf{0.18} & 0.26 & \textbf{0.31} \\
         \selfexp{} & 0.11 & 0.32 & 0.32 & 0.11 & 0.30 & 0.29 \\
         \selfexpk{} & 0.10 & \textbf{0.27} & 0.34 & 0.11 & \textbf{0.25} & \textbf{0.31} \\\bottomrule
    \end{tabular}
\end{table}
